Learning Dominant Wave Directions For Plane Wave Methods For High-Frequency Helmholtz Equations

We present a ray-based finite element method (ray-FEM) by learning basis adaptive to the underlying high-frequency Helmholtz equation in smooth media. Based on the geometric optics ansatz of the wave field, we learn local dominant ray directions by probing the medium using low-frequency waves with the same source. Once local ray directions are extracted, they are incorporated into the finite element basis to solve the high-frequency Helmholtz equation. This process can be continued to further improve approximations for both local ray directions and the high frequency wave field iteratively. The method requires a fixed number of grid points per wavelength to represent the wave field and achieves an asymptotic convergence as the frequency $\omega\rightarrow \infty$ without the pollution effect. A fast solver is developed for the resulting linear system with an empirical complexity $\mathcal{O}(\omega^d)$ up to a poly-logarithmic factor. Numerical examples in 2D are presented to corroborate the claims.

==> fast_solver.tex <==
%!TEX root = draft.tex

\section{Fast Linear Solver}

The main bottleneck, complexity-wise, in the computation fo the high-frequency Helmholtz equation is in the

The complexity estimates provided in Table \ref{tab:complexity} are based on the assumption that the linear system provided by both finite element formulations, standard P1 FEM and Ray-based FEM, which we write in a generic form as
\begin{equation} \label{eq:discrete_Helmholtz_equation}
\H\u = \f,
\end{equation}
can be solved in linear complexity (up to logarithmic factors).

This can be achieved using a variation of the method of polarized traces \cite{ZepedaDemanet:the_method_of_polarized_traces}, which we review shortly. The method of polarized traces is a domain decomposition method that encompasses the following aspects
\begin{itemize}
\item  layered domain decomposition;
\item  absorbing boundary conditions between subdomains implemented via PML \cite{Berenger:PML};
\item  transmission conditions issued from a discrete Green's representation formula;
\item  efficient preconditioner arising from localization of the waves via an incomplete Green's formula.
\end{itemize}

The first two aspects can be effortlessly implemented. Let consider a layered partition of $\Omega$ into $L$ slabs, or layers $\{ \Omega^{\ell} \}_{\ell =1}^{L}$. Define $f^{\ell}$ as the restriction of $f$ to $\Omega^{\ell}$, i.e., $f^{\ell} = f\chi_{\Omega^{\ell}}$; and define the local Helmholtz operators as
\begin{equation} \label{eq:local_Helmholtz}
\cH^{\ell} u  :=  \left( -\triangle  - m \omega^2  \right)  u   \qquad  \text{in } \Omega^{\ell},
\end{equation}
with absorbing boundary conditions implemented via PML between slabs.

The method of polarized traces aims to solve the global linear system in \eqref{eq:discrete_Helmholtz_equation}
by solving the local systems $\H^{\ell}$, which are the discrete version of \eqref{eq:local_Helmholtz}.

In order to solve the global system, or in this case to find a good approximate solution, we need to ``glue'' the subdomains together. This bring us to the third aspect of the method of polarized traces: the discrete Green's representation formula.

In the original formulation of the method of polarized traces \cite{ZepedaDemanet:the_method_of_polarized_traces}, the Green's representation formula was used to build a global  surface integral equation (SIE) at the interfaces between slabs. The SIE was solved using an efficient preconditioner coupled with a multilevel compression of the discrete kernels to accelerate the on-line stage of the algorithm. The original algorithm had superlinear off-line complexity which was amortized among a large number of right-hand sides, which represents a typical situation in explorations geophysics.

In the context of the present paper, the linear systems issued from the ray-based FEM depends on the right-hand side, making impossible to amortize a super-linear off-line cost. In order to reduce the off-line cost we use a matrix-free formulation (see Chapter 2 in \cite{Zepeda_Nunez:Fast_and_scalable_solvers_for_the_Helmholtz_equation}). Therefore, instead of providing the discrete Green's representation formula, we will seek an equivalent expression that will allows us to define the transmission conditions.

Given the geometrical connectivity between degrees of freedom in 2D, we have that $\H$ in \eqref{eq:discrete_Helmholtz_equation} can be written as
\begin{equation} \scriptsize \label{eq:Helmholtz_matrix}
    \H =    \left [ \begin{array}{cccccc}
                    \H_{1,1}    &  \H_{1,2}     &           &                   &       \\
                    \H_{2,1}    &  \H_{2,2}     &  \H_{2,3} &                   &       \\
                                &     \ddots    &   \ddots  & \ddots            &    \\
                                &               &    \ddots & \ddots            &   \H_{n_z-1, n_z}  \\
                                &               &           &   \H_{n_z, n_z-1} &   \H_{n_z,n_z}
                    \end{array}
            \right ],
\end{equation}
 in which all the sub-matrices are sparse. This particular representation induces an ordering of the unknowns
\begin{equation} \label{eq:global_ordering}
\u = (\u_1, \u_2, ..., \u_{n_z}),
\end{equation}
where $\u_j$ is a vector compatible with $\H_{j,j}$ in \eqref{eq:Helmholtz_matrix}.

In order to have a clearer exposition, we suppose that the mesh is structured as shown in Fig. \ref{fig:DD_Sketch}. Under that assumption, all the submatrices of $\H$ are square with the same size, allowing to use the notation
\begin{equation} \label{eq:trace_ordering}
\u_j = (u_{1,j}, u_{2,j},..., u_{n_x,j}),
\end{equation}
for the entries of $\u$ sampled at constant depth.

\begin{figure}[h]
\centering
\includegraphics[width=14cm]{pictures/DDM_sketch.pdf}
\caption{ The domain $\Omega$ is extended by adding the PML nodes (orange). After decompo-
sition into subdomains, the interfaces between subdomains are extended with PML nodes (light blue), finally the transmission conditions are imposed with artificial sources located at the red nodes.}
\label{fig:DD_Sketch}
\end{figure}


We write $\u^{\ell}$ for the wavefield defined locally at the $\ell$-th layer, i.e., $\u^{\ell}  = \chi_{\Omega^{\ell}}\u$, and $\u^{\ell}_k$ for the values at the local depth\footnote{We hope that there is little risk of confusion in overloading $z_{j}$ (local indexing) for $z_{n_c^{\ell} + j}$ (global indexing), where $n_c^{\ell} = \sum_{j=1}^{\ell-1} n^j$ is the cumulative number of points in depth.} $z_k^{\ell}$ of $\u^{\ell}$.

In particular, $\u^{\ell}_1$ represents the wavefield sampled at bottom of the slab, and  $\u^{\ell}_{n^{\ell}}$ is the wavefield at the top of the slab (see red nodes in Fig. \ref{fig:DD_Sketch} right-most picture). Moreover,  $\u^{\ell}_0$ is the local wavefield sampled immediately below the bottom of the slab, in the extended region within the PML; $\u^{\ell}_{n^{\ell}+1}$  is the local wavefield sampled immediately above the top of the slab.

Finally, we use the notation $\delta_{k}$ to denote a discrete measure. For a generic vector $ \mathbf{p} \in \CC^{n_x}$,   $\delta_{k} \mathbf{p} \in \CC^{n_x\times n_z}$ is defined as follows:
\begin{equation}
    (\delta_{k} \mathbf{p})_{i,j} = \left \{  \begin{array}{cl}
                                    \mathbf{p}_i & \mbox{if } j = k,  \\
                                    0        & \mbox{if } j\neq k.
                            \end{array} \right .
 \end{equation}
This notation will be used extensively to characterize the forcing terms necessary to transfer the information from one subdomain to its neighbors.

In order to keep the presentation as clean as possible, we only present the correct formula and we redirect the interested reader to Chapter 2 of \cite{Zepeda_Nunez:Fast_and_scalable_solvers_for_the_Helmholtz_equation} for further details. We can then use the same approach as in \cite{Zepeda_Nunez:Fast_and_scalable_solvers_for_the_Helmholtz_equation} to obtain the discrete Green's representation formula.

 The correct Green's representation formula is given by the equivalent and more manageable expression \footnote{It is possible to recover the Green's representation formula by multiplying \eqref{eq:pde_GRF_real} by the inverse of $ \H^{\ell} $}
 \begin{align} \label{eq:pde_GRF_real}
    \H^{\ell} \v^{\ell} =  & - \delta_{n^{\ell}} \H^{\ell}_{n^{\ell},n^{\ell}+1} \u_{n^{\ell}+1}  +  \delta_{n^{\ell}+1}  \H^{\ell}_{n^{\ell}+1,n^{\ell}} \u_{n^{\ell}} \\
    & -  \delta_{1}  \H^{\ell}_{1,0} \u_{0}  + \delta_{0}  \H^{\ell}_{0,1} \u_{1} + \f^{\ell} . \nonumber
\end{align}

Finally, we can discuss the last aspect of the preconditioner, which is the localization of the waves and the preconditioner.

The main idea of the localization of the waves, is that the absorbing boundary conditions provides a direction to the waves. For example, the wavefield generated by a local source,
\begin{equation}
\H^{\ell} \v^{\ell} = \f^{\ell},
\end{equation}
irradiates from the interior of $\Omega^{\ell}$, where the source is non-zero, to the exterior of it. If we sample $\v^{\ell}$ at the bottom of $\Omega^{\ell}$, we can physically interpret it as the trace of a wavefield propagating downwards. Analogously, if we sample $\v^{\ell}$ at the top of $\Omega^{\ell}$, we can interpret it as a trace of a wavefield propagating upwards.

Following with the physical interpretation, the wavefield propagating downwards from $\Omega^{\ell}$ should propagate inwards $\Omega^{\ell-1}$. We can then propagate the wavefield from $\Omega^{\ell}$ in $\Omega^{\ell-1}$ by artificial sources located at the top of $\Omega^{\ell-1}$. The resulting expression is given by
\begin{align} \label{eq:pde_GRF_down}
    \H^{\ell-1} \v^{\ell-1} =  & - \delta_{n^{\ell-1}} \H^{\ell-1}_{n^{\ell-1},n^{\ell-1}+1} \v^{\ell}_{1}  +  \delta_{n^{\ell-1}+1}  \H^{\ell-1}_{n^{\ell-1}+1,n^{\ell-1}}  \v^{\ell}_{0}  + \f^{\ell-1},
\end{align}
which is an alternate expression for the incomplete Green's representation formula introduced in \cite{ZepedaDemanet:the_method_of_polarized_traces}. For a more complete exposition please see Section 1.1 in \cite{ZepedaDemanet:the_method_of_polarized_traces}.

We can observe that $\v^{\ell-1} $ contains the energy radiating from $\f^{\ell-1}$ and $\f^{\ell}$, in  which the last is given by the extra sources at the top interface. If we sample $\v^{\ell-1}$ at the bottom of $\Omega^{\ell-1}$, it can be interpreted as the downwards wavefield consisting on the downwards wavefield generated by $\f^{\ell-1}$ and the wavefield generated by $\f^{\ell}$ that propagated through $\Omega^{\ell-1}$.

We can continue the propagation adding the local downwards wavefields in a manner that is usually called a multiplicative Schwarz iteration. Analogously, the same procedure can be performed for the wavefields propagating upwards, resulting in the polarized traces preconditioner as shown in Alg. \ref{alg:GS_preconditioner}. We point out that an extra step is added in the upward pass to decrease the number of iterations.

All the intuitive arguments provided in the current exposition can be made rigorous from an algebraic point of view, we skip such an explanation but we redirect the interested reader to \cite{ZepedaDemanet:the_method_of_polarized_traces}.

% In the original method of polarized trace the SIE is solved first using preconditioned GMRES, and then the wavefield is locally reconstructed in the volume via the GRF. In the present work, we precondition the equation in the volume in a way that is reminiscent of the sweeping preconditioner \cite{EngquistYing:Sweeping_PML} and the rapidly convergent domain decomposition \cite{CStolk_rapidily_converging_domain_decomposition}.

Finally, we solve \eqref{eq:discrete_Helmholtz_equation} using GMRES left-preconditioned with Alg. \ref{alg:GS_preconditioner}.

\begin{algorithm} Gauss-Seidel Preconditioner \label{alg:GS_preconditioner}
    \begin{algorithmic}[h]
        \Function{ $\u$ = Preconditioner}{ $\f$ }
            \For{  $\ell = 1: L$ } \Comment{Downwards Sweep}
                \State $ \f^{\ell} = \f \chi_{\Omega^{\ell}} $ \Comment{Partition of the Source}
                \If{ $\ell \neq 1$ }
                %\State $ \f^{\ell} = \f^{\ell} - \delta_{1}  \H^{\ell}_{1,0} \u_{0}  + \delta_{0}  \H^{\ell}_{0,1} \u_{1} $
                \State $ \f^{\ell} $+=$  - \delta_{n^{\ell}} \H^{\ell}_{n^{\ell},n^{\ell}+1} \mathbf{w}^{\ell-1}_{1}  +  \delta_{n^{\ell}+1}  \H^{\ell}_{n^{\ell}+1,n^{\ell}}  \mathbf{w}^{\ell-1}_{0}  $
                \EndIf
                \State $\mathbf{w}^{\ell}  = (\mathbf{H}^{\ell})^{-1}\f^{\ell}$
            \EndFor

            \For{  $\ell = L:-1:1$ } \Comment{Upwards Sweep}
                \State $ \f^{\ell} = \f \chi_{\Omega^{\ell}} $ \Comment{Partition of the Source}
                \If{ $\ell \neq L$ }
                %\State $ \f^{\ell} = \f^{\ell} - \delta_{1}  \H^{\ell}_{1,0} \u_{0}  + \delta_{0}  \H^{\ell}_{0,1} \u_{1} $
                \State $ \f^{\ell} += - \delta_{1} \H^{\ell}_{1,0} \u^{\ell+1}_{n^{\ell}}  + \delta_{0}  \H^{\ell}_{0,1} \u^{\ell+1}_{n^{\ell}+1} $
                \EndIf

                \If{ $\ell \neq 1$ }
                %\State $ \f^{\ell} = \f^{\ell} - \delta_{1}  \H^{\ell}_{1,0} \u_{0}  + \delta_{0}  \H^{\ell}_{0,1} \u_{1} $
                \State $ \f^{\ell} +=  - \delta_{n^{\ell}} \H^{\ell}_{n^{\ell},n^{\ell}+1} \mathbf{w}^{\ell-1}_{1}  +  \delta_{n^{\ell}+1}  \H^{\ell}_{n^{\ell}+1,n^{\ell}}  \mathbf{w}^{\ell-1}_{0}  $
                \EndIf
                \State $\u^{\ell}  = (\mathbf{H}^{\ell})^{-1}\f^{\ell}$
            \EndFor

            \State $\u =  \left (\u^{1}, \u^{2}, \u^{3}, ..., \u^{L-1}, \u^{L}  \right)$ \Comment{Concatenation}
        \EndFunction
    \end{algorithmic}
\end{algorithm}


\subsection{Complexity}

The method explained is a powerful framework to develop domain decomposition method for wave propagation. In general, the number of iteration for convergence will depend on the quality of the absorbing boundary conditions, and the wavespeed. In the best case, the number of iterations will depend on the number of physical reflections.

For a smooth and fixed wave-speed, several numerical experiments indicate that the number of iterations to convergence is independent of the frequency. Meaning that the cost is dominate by the factorization and solve of each local linear system.

If we suppose that $\Omega$ is discretized in $N = n^2$ elements, and that each slab is only $\cO(1)$ elements thick, then we have that factorizing all the local problems using a multifrontal method \cite{Duff_Reid:The_Multifrontal_Solution_of_Indefinite_Sparse_Symmetric_Linear,GeorgeNested_dissection} (in this case UMFPACK \cite{Davis:UMFPACK}) will have an asymptotic cost of $\cO(n)$, which has to be performed $\cO(n)$ times, leading to an off-line cost of $\cO(N)$

For the online stage (Alg. \ref{alg:GS_preconditioner}) we need to solve $\cO(n)$ quasi 1-D linear systems, which can be performed in $\cO(n)$ time, leading to a $\cO(N)$ complexity for each iteration. Finally, given that the number of iterations are $\cO(1)$ we have a linear overall complexity.

We point out, that this method can be seamlessly extended to 3D, where the complexity will be $\cO(N^{4/3})$ for the off-line part and $\cO(N\log(N))$ for the on-line stage. Moreover, a nested sweep technique can be implemented in 3D \cite{Liu_Ying:Recursive_sweeping_preconditioner_for_the_3d_helmholtz_equation,Zepeda_Nunez:Fast_and_scalable_solvers_for_the_Helmholtz_equation} that can bring the asymptotic cost to  $\cO(N)$ for the off-line part and $\cO(N)$ for the on-line stage, albeit with larger constants.


